AccuQuant: Simulating Multiple Denoising Steps for Quantizing Diffusion Models

We present in this paper a novel post-training quantization (PTQ) method, dubbed AccuQuant, for diffusion models. We show analytically and empirically that quantization errors for diffusion models are accumulated over denoising steps in a sampling process. To alleviate the error accumulation problem, AccuQuant minimizes the discrepancies between outputs of a full-precision diffusion model and its quantized version within a couple of denoising steps. That is, it simulates multiple denoising steps of a diffusion sampling process explicitly for quantization, accounting the accumulated errors over multiple denoising steps, which is in contrast to previous approaches to imitating a training process of diffusion models, namely, minimizing the discrepancies independently for each step. We also present an efficient implementation technique for AccuQuant, together with a novel objective, which reduces a memory complexity significantly from $\mathcal{O}(n)$ to $\mathcal{O}(1)$, where $n$ is the number of denoising steps. We demonstrate the efficacy and efficiency of AccuQuant across various tasks and diffusion models on standard benchmarks.

==> accuquant-neurips-cameraready-arxiv/fig/quali_coco.tex <==
\begin{figure*}[!t]
  \vspace{2mm}

   \captionsetup[subfigure]{font=small, labelformat=empty}
   \begin{center}
     % Full-Precision
     \begin{subfigure}[c]{0.24\linewidth}
       \centering
       \begin{tabular}{c @{\hspace{0.5mm}} c}
         \includegraphics[width=0.48\columnwidth]{fig/coco/fp/00027.pdf} &
         \includegraphics[width=0.48\columnwidth]{fig/coco/fp/00128.pdf} \\
         \includegraphics[width=0.48\columnwidth]{fig/coco/fp/00075.pdf} &
         \includegraphics[width=0.48\columnwidth]{fig/coco/fp/00253.pdf} \\
       \end{tabular}
       \label{fig:fp}
       \vspace{-3mm}
       \caption{Full-Precision}
     \end{subfigure}
     \hfill
     \begin{subfigure}[c]{0.24\linewidth}
      \centering
      \begin{tabular}{c @{\hspace{0.5mm}} c}
        \includegraphics[width=0.48\columnwidth]{fig/coco/qdiff/00027.pdf} &
        \includegraphics[width=0.48\columnwidth]{fig/coco/qdiff/00128.pdf} \\
        \includegraphics[width=0.48\columnwidth]{fig/coco/qdiff/00075.pdf} &
        \includegraphics[width=0.48\columnwidth]{fig/coco/qdiff/00253.pdf} \\
      \end{tabular}
      \label{fig:qdiff}
      \vspace{-3mm}
      \caption{Q-Diffusion~\cite{li2023q}}
    \end{subfigure}
    \hfill
    % PCR (τ=0.2)     % pcr
     \begin{subfigure}[c]{0.24\linewidth}
       \centering
       \begin{tabular}{c @{\hspace{0.5mm}} c}
         \includegraphics[width=0.48\columnwidth]{fig/coco/pcr/00027.pdf} &
         \includegraphics[width=0.48\columnwidth]{fig/coco/pcr/00128.pdf} \\
         \includegraphics[width=0.48\columnwidth]{fig/coco/pcr/00075.pdf} &
         \includegraphics[width=0.48\columnwidth]{fig/coco/pcr/00253.pdf} \\
       \end{tabular}
       \label{fig:pcr}
       \vspace{-3mm}
       \caption{PCR ($\tau=0.20$)~\cite{tang2025post}}
     \end{subfigure}
     \hfill
     % Q-Diffusion
     \begin{subfigure}[c]{0.24\linewidth}
      \centering
      \begin{tabular}{c @{\hspace{0.5mm}} c}
        \includegraphics[width=0.48\columnwidth]{fig/coco/ours/00027.pdf} &
        \includegraphics[width=0.48\columnwidth]{fig/coco/ours/00128.pdf} \\
        \includegraphics[width=0.48\columnwidth]{fig/coco/ours/00075.pdf} &
        \includegraphics[width=0.48\columnwidth]{fig/coco/ours/00253.pdf} \\
      \end{tabular}
      \label{fig:ours}
      \vspace{-3mm}
      \caption{Ours}
     \end{subfigure}
   \end{center}
   \vspace{-3mm}
   \caption{Visual comparisons of generated images conditioned on text prompts. We generate images by SD v1.4~\cite{rombach2022high} and its quantized versions using PCR~\cite{tang2025post} under a 4/8.4-bit setting and Q-Diffusion~\cite{li2023q}, AccuQuant under a 4/8-bit setting. $\tau=0.20$ indicates setting 20\% of entire denoising steps into 10 bits. The prompts corresponding to each column are: \textit{``A puppy wearing a hat"} and \textit{``A cute teddy bear in front of a plain wall, warm and brown fur."}}
   \vspace{-3mm}
   
   \label{fig:sd_results_updated}
 \end{figure*}



==> accuquant-neurips-cameraready-arxiv/fig/quali_grad_memory.tex <==
\begin{figure}[!t]
    \vspace{-1mm}        
    \centering
    \includegraphics[width=0.6\linewidth]{./fig/grad_memory.pdf}
    \vspace{-1mm}        
    \caption{Comparisons of a total amount of memory of AccuQuant with and without the gradient approximation. We measure the memory usage during the calibration process of AccuQuant under a 6/6-bit setting for DDIM~\cite{song2020denoising} on CIFAR-10~\cite{krizhevsky2009learning}.}
    \label{fig:grad_memory}
    \vspace{-2mm}        
\end{figure}


==> accuquant-neurips-cameraready-arxiv/fig/quali_groupsize.tex <==

\begin{figure*}[!t]
    \centering
    \captionsetup[subfigure]{font=small, labelformat=empty}
    
    \begin{subfigure}[c]{1.0\linewidth}
       \centering
       \begin{tabular}{c @{} c @{} c @{} c @{} c @{} c @{} c @{} c @{} c}
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/74.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/1.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/3.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/10.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/11.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/28.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/30.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/34.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/fp/cifar10/56.pdf} \\
       \end{tabular}
    \end{subfigure}
    \vspace{-1.5mm}

    \begin{subfigure}[c]{1.0\linewidth}
       \centering
       \begin{tabular}{c @{} c @{} c @{} c @{} c @{} c @{} c @{} c @{} c}
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/74.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/1.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/3.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/10.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/11.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/28.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/30.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/34.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group1/56.pdf} \\
       \end{tabular}
    \end{subfigure}
    \vspace{-1.5mm}

    \begin{subfigure}[c]{1.0\linewidth}
       \centering
       \begin{tabular}{c @{} c @{} c @{} c @{} c @{} c @{} c @{} c @{} c}
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/74.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/1.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/3.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/10.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/11.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/28.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/30.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/34.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group5/56.pdf} \\
       \end{tabular}
    \end{subfigure}
    \vspace{-1.5mm}

    \begin{subfigure}[c]{1.0\linewidth}
       \centering
       \begin{tabular}{c @{} c @{} c @{} c @{} c @{} c @{} c @{} c @{} c}
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/74.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/1.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/3.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/10.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/11.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/28.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/30.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/34.pdf} &
          \includegraphics[width=0.1\linewidth]{fig/fig_quali/ours/cifar10/group100/56.pdf} \\
       \end{tabular}
    \end{subfigure}
    \vspace{-1.5mm}
    
    \caption{Visual comparisons of DDIM~\cite{song2020denoising} for unconditional image generation on CIFAR-10~\cite{krizhevsky2009learning} under various group sizes. Both weights and activations were quantized to 6 bits for a visually distinct and clear comparison. From top to bottom, the presented sequences correspond to the full-precision model, our method with group sizes of 1, 5, and 100.}
    \label{fig:quali_groupsize}
    \vspace{-5mm}
\end{figure*}


==> accuquant-neurips-cameraready-arxiv/fig/quali_lsun.tex <==
\begin{figure*}[!t]
   \vspace{2mm}
   \captionsetup[subfigure]{font=small, labelformat=empty}
   \begin{center}
   \begin{subfigure}[c]{0.24\linewidth}
      \centering
      % \fbox{\rule{0in}{1in} \rule{1.5in}{0in}}
      \begin{tabular}{c @{\hspace{0.5mm}} c @{\hspace{0.5mm}} c}
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/fp/bedroom/1.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/fp/bedroom/2.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/fp/bedroom/3.pdf}\\
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/fp/church/1.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/fp/church/2.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/fp/church/3.pdf}\\
      \end{tabular}
      \label{fig:lsun_fp}
      \vspace{-3mm}
      \caption{Full precision}
   \end{subfigure}
   \begin{subfigure}[c]{0.24\linewidth}
      \centering
      \begin{tabular}{c @{\hspace{0.5mm}} c @{\hspace{0.5mm}} c}
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/qdiff/bedroom/1.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/qdiff/bedroom/2.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/qdiff/bedroom/3.pdf}\\
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/qdiff/church/1.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/qdiff/church/2.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/qdiff/church/3.pdf}\\
      \end{tabular}
      \label{fig:lsun_qdiff}
      \vspace{-3mm}
      \caption{Q-Diffusion~\cite{li2023q}}
   \end{subfigure}
   \begin{subfigure}[c]{0.24\linewidth}
      \centering
      \begin{tabular}{c @{\hspace{0.5mm}} c @{\hspace{0.5mm}} c}
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/tfmq/bedroom/1.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/tfmq/bedroom/2.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/tfmq/bedroom/3.pdf}\\
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/tfmq/church/1.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/tfmq/church/2.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/tfmq/church/3.pdf}\\
      \end{tabular}
      \label{fig:lsun_tfmq}
      \vspace{-3mm}
      \caption{TFMQ-DM~\cite{huang2024tfmq}}
   \end{subfigure}
   \begin{subfigure}[c]{0.24\linewidth}
      \centering
      \begin{tabular}{c @{\hspace{0.5mm}} c @{\hspace{0.5mm}} c}
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/ours/bedroom/1.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/ours/bedroom/2.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/ours/bedroom/3.pdf}\\
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/ours/church/1.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/ours/church/2.pdf}&
         \includegraphics[width=0.3\columnwidth]{fig/fig_quali/ours/church/3.pdf}\\
      \end{tabular}
      \label{fig:lsun_ours}
      \vspace{-3mm}
      \caption{Ours}
   \end{subfigure}
   \vspace{-2mm}
   \caption{Visual comparisons of generated images on (\textbf{Top})~LSUN-Bedrooms~\cite{yu2015lsun} and (\textbf{Bottom})~LSUN-Churches~\cite{yu2015lsun} for unconditional image generation under a 3/8-bit setting.}
   \label{fig:lsun_results}
   \end{center}
   \vspace{-3mm}
 \end{figure*}

 

==> accuquant-neurips-cameraready-arxiv/supple.tex <==
\section{Detailed algorithm for AccuQuant}
\label{appendix:algorithm}
\subsection{Algorithm table for AccuQuant}
\vspace{-10mm}
\begin{algorithm}
\caption{Pseudo code of AccuQuant.}
\label{alg:accuquant}
\begin{lstlisting}[language=Python]
# M : group size
# x_T : random gaussian noise
# fp_model : full-precision model
# quant_model : quantized model
# gather_output() : one iteration of diffusion denoising step
# sg() : stop gradient operation

# Initialize
x_t = x_T
t = T
group_index = 0

for i in range(number_of_groups):
    # Gather x_(t-M) from Full Precision Model
    with torch.no_grad():
        fp_x_M = gather_output(fp_model,x_t,t)

    # Reconstruction stage
    quant_model.set_group(group_index)
    optimizer=torch.optim.Adam(quant_params,learning_rate)

    for epoch in range(epochs):
        # Gather \tilde x_(t-M) with stop gradient
        with torch.no_grad():
            sg_quant_x_M = gather_output(quant_model,x_m,m,quant_params)
        
        optimizer.zero_grad()

        # Accumulate the gradient
        for m in range(M):
            # Calculate gradient scaling factor
            g_m =sqrt_alpha_M / sqrt_alpha_m

            # Gather \tilde x_(t-m)
            quant_x_m = gather_output(quant_model,x_m,m,quant_params)

            # Compute \tilde x_(t-M) with stop gradient
            quant_x_M = sg_quant_x_M - sg(quant_x_m) + quant_x_m

            # Compute Loss for current step
            loss_accuquant = torch.mse(fp_x_M - quant_x_M) * g_m

            # Update quantization parameters with accumulated gradients
            loss_accuquant.backward()
        
        optimizer.step()

    # update indices
    x_t = fp_x_M
    t = t-M
    group_index += 1
\end{lstlisting}
\end{algorithm}
    
\subsection{Detailed derivations of Eq.~\eqref{eq:gradient_approximation}}
\label{appendix:gm_proof}

We provide a detailed derivation of Eq.~\eqref{eq:gradient_approximation}. We can represent the gradient between consecutive denoising steps for the quantized diffusion model as follows:
\begin{equation}
    \frac{\partial \tilde{x}_{t-1}}{\partial \tilde{x}_{t}} = \frac{\sqrt{\alpha_{t-1}}}{\sqrt{\alpha_{t}}}I+\left( -\frac{\sqrt{\alpha_{t-1}}\sqrt{1-\alpha_{t}}}{\sqrt{\alpha_{t}}} + \sqrt{1-\alpha_{t-1}} \right) \frac{\partial \tilde{\epsilon}_\theta(\tilde{x}_t,t)}{\partial \tilde{x}_{t}}.
    \label{eq:real_gradient_supple}
\end{equation}
Here, $I$ is the identity matrix, and $\tilde{\epsilon}_\theta(\tilde{x}_t,t)$ is the output of the quantized model. We have empirically observed in Fig.~\ref{fig:gradient_approximation} that the first term in~Eq.~\eqref{eq:real_gradient} dominates the entire gradient, whereas the second one is negligible. Based on this observation, we approximate the gradient in Eq.~\eqref{eq:real_gradient} by omitting the second term as follows:
\begin{equation} 
    \frac{\partial \tilde{x}_{t-1}}{\partial \tilde{x}_{t}} \approx \frac{\sqrt{\alpha_{t-1}}}{\sqrt{\alpha_{t}}}I. \label{eq:appendix_grad} 
\end{equation}
Using Eq.~\eqref{eq:appendix_grad} in Eq.~\eqref{eq:g_m_approximation}, we obtain the approximated $g_m$ as follows:
\begin{align} 
    g_m &= 
    \begin{cases} 
        1 & m = M \\ 
        \prod_{j=1}^{M-m}\frac{\partial \tilde{x}_{{t}-M-1+j}}{\partial \tilde{x}_{{t}-M+j}}, & m \neq M, 
    \end{cases}\\
    &\approx
    \begin{cases} 
        1 & m = M \\ 
        \prod_{j=1}^{M-m}\frac{\partial x_{{t}-M-1+j}}{\partial x_{{t}-M+j}}, & m \neq M, 
    \end{cases}\\
    &\approx    
    \begin{cases} 
        1 & m = M \\
        \prod_{j=1}^{M-m}\frac{\sqrt{\alpha_{t-M-1+j}}}{\sqrt{\alpha_{t-M+j}}}I, & m \neq M, 
    \end{cases}\\
    &= \frac{\sqrt{\alpha_{t-M}}}{\sqrt{\alpha_{t-m}}}I, \quad \text{for } m = 1,2,\dots,M. \label{eq:appendix_g_m} 
\end{align}


\subsection{Detailed derivation of the objective in Eq.~\eqref{eq:AccuQuantloss} with the gradient approximation}
\label{appendix:loss_proof}
We derive a loss function in Eq.~\eqref{eq:AccuQuantloss} incorporating our gradient approximation of Eq.~\eqref{eq:appendix_g_m}. First, by substituting Eq.\eqref{eq:appendix_g_m} into Eq.~\eqref{eq:group_gradient}, we obtain:
\begin{align} 
    \frac{\partial \mathcal{L}_{\text{MSE}}}{\partial s_l} 
    &= \frac{\partial\mathcal{L}_{\text{MSE}}}{\partial \tilde{x}_{{t}-M}} \left[\sum_{m=1}^{M} g_m \frac{\partial \tilde{x}_{{t}-m}}{\partial s_l} \right] \\
    &\approx \frac{\partial\mathcal{L}_{\text{MSE}}}{\partial \tilde{x}_{{t}-M}} \left[\sum_{m=1}^{M} \frac{\sqrt{\alpha_{t-M}}}{\sqrt{\alpha_{t-m}}} \frac{\partial \tilde{x}_{{t}-m}}{\partial s_l} \right]\\
    &= 2 (\tilde{x}_{t-M} - x_{t-M})^\top \left[\sum_{m=1}^{M} \frac{\sqrt{\alpha_{t-M}}}{\sqrt{\alpha_{t-m}}} \frac{\partial \tilde{x}_{{t}-m}}{\partial s_l} \right] \\
    &= \sum_{m=1}^{M} \frac{\sqrt{\alpha_{t-M}}}{\sqrt{\alpha_{t-m}}} \left[ 2(\tilde{x}_{t-M} - x_{t-M})^\top \frac{\partial \tilde{x}_{{t}-m}}{\partial s_l} \right]. 
    \label{eq:appendix_group_gradient} 
\end{align}
Note that we omit identity matrix in Eq.~\eqref{eq:appendix_g_m} for simple notation. From Eq.~\eqref{eq:appendix_group_gradient}, we derive a loss function whose gradient matches the derived expression by adding $x_{t-m}$ and subtracting a detached version of $x_{t-m}$ within the squared term:
\begin{equation}
    \mathcal{L}_{\text{AccuQuant}} = \sum_{m=1}^{M} \frac{\sqrt{\alpha_{t-M}}}{\sqrt{\alpha_{t-m}}} \lVert \texttt{sg}(x_{t-M} - \tilde{x}_{t-M}) + \tilde{x}_{t-m} - \texttt{sg}(\tilde{x}_{t-m})\rVert_2^2 .
    \label{eq:appendix_loss}
\end{equation}
In this formulation, we compute $x_{t-M}$ and $\tilde{x}_{t-M}$ before updating gradients without saving intermediate feature maps and treat it as a constant during optimization. We then compute loss term inside the summation and accumulate its gradients progressively over multiple denoising steps. After completing $M$ denoising steps, we update the step size using the cumulative gradient. The detailed pipeline of our method is provided in Algorithm~\ref{alg:accuquant}.

\section{Implementation details}
\label{sec:details_appendix}
For weight quantization, we adopt a uniform quantizer identical for all denoising steps, following Q-Diffusion~\cite{li2023q}, since the weights remain invariant across different denoising steps. 
For the CIFAR-10~\cite{krizhevsky2009learning}, we employ the DDIM~\cite{song2020denoising} with 100 total denoising steps, grouping them into 20 sets of 5 denoising steps each and setting learning rate in $\{1\times10^{-3},\,4\times10^{-4}\}$. For the LSUN-Bedroom~\cite{yu2015lsun}, we use LDM-4~\cite{rombach2022high} and the DDIM sampler~\cite{song2020denoising} with 200 total denoising steps, grouping them into 20 sets of 10 denoising steps each and setting learning rate into $4\times10^{-5}$. For the LSUN-Church~\cite{yu2015lsun}, we use LDM-8~\cite{rombach2022high} and the DDIM sampler~\cite{song2020denoising} with 500 total denoising steps, grouping them into 20 sets of 25 denoising steps each and setting learning rate into $4\times10^{-5}$. For the ImageNet~\cite{deng2009imagenet}, we employ LDM-4~\cite{rombach2022high} and the DDIM sampler~\cite{song2020denoising} with 20 total denoising steps and forming 10 groups and setting learning rate into $1\times10^{-3}$. For text-to-image generation, we employ Stable-Diffusion v1.4~\footnote{\url{https://huggingface.co/CompVis/stable-diffusion-v-1-4-original}\label{fn:sd}} with the PNDM sampler~\cite{liu2022pseudo}, using 50 total denoising steps and forming 25 groups and setting learning rate into $1\times10^{-5}$. We set the calibration batch size to 8 for DDIM~\cite{song2020denoising} and LDMs~\cite{rombach2022high}, and to 1 for Stable Diffusion~\cite{rombach2022high}. All other experimental settings are identical to those of Q-Diffusion~\cite{li2023q}. We also retain the default settings~\cite{rombach2022high} during the sampling phase, ensuring that we can conduct all experiments on a single A100~(80 GB) GPU. Also, to ensure a fair comparison, we quantize every layer of TFMQ-DM~\cite{huang2024tfmq}, such as attention-modules and skip-connections for unconditional image generation. Finally, we evaluate the FID~\cite{heusel2017gans} and IS~\cite{salimans2016improved} scores, including the FID2FP32 metric~\cite{tang2025post}, using the torch-fidelity library~\footnote{\url{https://github.com/toshas/torch-fidelity}} and the official Guided Diffusion~\cite{dhariwal2021diffusion} codebase.

\section{Detailed analysis of quantitative results}
In this section, we analyze the quantitative results presented in Tables 1–3.
Firstly, Table 1 shows that AccuQuant outperforms other methods in most settings. In particular, AccuQuant achieves overwhelmingly superior performance on the FID2FP32~\cite{tang2025post} metric across all bit-widths, and this effect becomes more pronounced at lower bit-widths~(\textit{\eg, 3/6 bits}). Furthermore, AccuQuant achieves higher scores on the FID~\cite{heusel2017gans}, sFID~\cite{nash2021generating}, and IS~\cite{salimans2016improved} metrics compared to previous methods~\cite{li2023q,huang2024tfmq,yao2024timestep}, which are not designed for reducing the accumulated quantization error. These findings indicate that AccuQuant effectively reduces accumulated quantization error allowing better performance and confirms that minimizing the accumulated quantization error constitutes a crucial factor in diffusion model quantization.
Secondly, for the class-conditional image generation task reported in Table 2, we draw on previous work~\cite{yao2024timestep} showing that FID~\cite{heusel2017gans} does not perform reliably on ImageNet~\cite{deng2009imagenet} and therefore we report LPIPS~\cite{zhang2018unreasonable}, PSNR, and SSIM metrics to quantify differences between the full precision and quantized models. Likewise to FID2FP32~\cite{tang2025post}, these metrics measure how closely the quantized model’s outputs match those of the full precision model. We find that AccuQuant outperforms previous methods in terms of FID2FP32~\cite{tang2025post}, LPIPS~\cite{zhang2018unreasonable}, PSNR, and SSIM across all bit-widths, demonstrating that AccuQuant generates images that most closely resemble the full precision model’s outputs while maintaining high visual quality. These results imply that accumulated quantization error remains critical even when employing few denoising steps, such as 20. Furthermore, even compared to PTQD~\cite{he2023ptqd}, which is designed to reduce accumulating quantization error, AccuQuant outperforms it in FID2FP32~\cite{tang2025post}, LPIPS~\cite{zhang2018unreasonable}, PSNR, and SSIM across all bit widths, demonstrating the superiority of our framework in explicitly reducing accumulating quantization error.
Finally, the text-to-image generation results in Table 3 reveal that, despite PCR~\cite{tang2025post} use of more bit-widths~(\textit{\ie,} 8.4 bits for activations) and adopting independent quantizer at every denoising steps, AccuQuant achieves a better FID2FP32~\cite{tang2025post} score. Additionally, AccuQuant attains the highest CLIP-Score~\cite{hessel2022clipscore}, indicating that it not only reproduces images similar to the full precision model but also aligns them effectively with the text prompts.
To this end, our findings demonstrate that the AccuQuant framework outperforms existing methods for reducing accumulated quantization error, and that AccuQuant not only achieves results comparable to those of the full-precision model but also confirms the fidelity term by resulting superior performance on FID~\cite{heusel2017gans}, sFID~\cite{nash2021generating}, and CLIP score~\cite{hessel2022clipscore}.

\input{fig/quali_groupsize.tex}
\section{Qualitative results for group sizes}
In this section, we present the qualitative results for various group sizes, as reported in Table~\ref{tab:group_size}. We observe from Fig.~\ref{fig:quali_groupsize} that selecting an appropriate group size (e.g., group size of 5) generate images that closely resembling those of the full-precision model, under low bit-widhts.
 For example, in the first row of generated horse images, we can see that when the group size is set to 1, the quantized model fails to adequately account for accumulated errors, leading to the generation of distorted and unrealistic shapes. Similarly, when the group size is excessively large (e.g., group size of 100), the quantized model is unable to effectively manage the substantial accumulation of errors, resulting in unrealistic image outputs. In contrast, with an appropriately chosen group size (e.g., group size of 5), the accumulated errors are effectively mitigated, allowing the generated images to maintain a structure and appearance comparable to those of the full-precision model. In the dog images of column 6, using a group size of 5 yields images that most closely match the full-precision model in both texture and shape, outperforming group sizes 1 and 100. This indicates that an appropriate group sizes is a crucial factor to mitigate the accumulating quantization error.

 \input{tab/ablation_groupgrad.tex}
 \input{fig/quali_grad_memory.tex} 
\section{Quantitative results for group sizes and gradient approximation}
In this section, we show in Table.~\ref{tab:ablation_groupgrad} quantitative ablation results for varying group sizes, both with and without gradient approximation, for 4/8-bit quantized DDIM~\cite{song2020denoising} on CIFAR-10~\cite{krizhevsky2009learning}. We observe that both FID~\cite{heusel2017gans} and FID2FP32~\cite{tang2025post} degrade at group sizes of 1 and 25, since a group size of 1 fails to capture accumulated quantization error, whereas 25 is too large to find quantization parameters minimizing the error. This result highlights the importance of selecting appropriate group sizes and aligns with the findings discussed in the main paper. We also investigate the impact of gradient approximation. When the group size is 1, we calculate the gradient at every denoising steps and therefore the approximation has no effect on performance. We show that using gradient approximation usually yields better performance, since the gradients of Eq.~\eqref{eq:real_gradient} are corrupted before the quantization parameters $s_l$ converge, leading unstable calibration process. We also show in Fig.~\ref{fig:grad_memory} a total amount of memory of AccuQuant with and without the gradient approximation, \wrt the group size. The results show that the memory requirement grows linearly with group size in the absence of the gradient approximation, whereas it remains constant across all group sizes when the approximation is applied. Consequently, omitting the noisy gradient term effectively reduce memory requirement and ensure calibration process stable.

\begin{figure*}[!t]
    \centering
    \captionsetup[subfigure]{font=small, labelformat=empty, justification=centering}
    \captionsetup{justification=raggedright, singlelinecheck=false}

    \begin{subfigure}[t]{0.48\textwidth}
      \centering
      \makebox[0pt][l]{\hspace*{-36mm}\includegraphics[width=\linewidth]{fig/grad_bedroom.pdf}}
      \caption{LSUN-Bedroom}
      \label{fig:grad_bedroom}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
      \centering
      \makebox[0pt][l]{\hspace*{-37mm}\includegraphics[width=\linewidth]{fig/grad_church.pdf}}

      \caption{LSUN-Church}
      \label{fig:grad_church}
    \end{subfigure}

    \caption{Plots of the gradient in Eq.~\eqref{eq:real_gradient_supple} and its components over denoising steps. The gradients are calculated during a calibration process of AccuQuant for LSUN-Bedroom~\cite{yu2015lsun} on the left and LSUN-Church~\cite{yu2015lsun} on the right.}
    \label{fig:gradients_bedroom_church}
\end{figure*}

\section{Gradient approximation across different dataset}
In this section, we visualize the gradient approximation on LDM-4 and LDM-8~\cite{rombach2022high} across diverse datasets, including LSUN-Bedroom and LSUN-Church~\cite{yu2015lsun}, as illustrated in Fig.~\ref{fig:gradients_bedroom_church}. We plot the full gradients of Eq.~\eqref{eq:real_gradient_supple}, the gradient approximation of Eq.~\eqref{eq:appendix_grad}, and the residual term~(\textit{\ie}, $c_t\frac{\partial \tilde{\epsilon}_\theta(\tilde{x}_t,t)}{\partial \tilde{x}_{t}}$) at 200 and 500 denoising steps. The results show that, consistent with the behavior observed in Fig.~\ref{fig:gradients_bedroom_church}, the gradient approximation remains closely aligned with the full gradient throughout multiple denoising steps on both datasets, thereby corroborating the validity of our approximation. Moreover, as discussed in Table.~\ref{tab:grad_approx} and Table.~\ref{tab:ablation_groupgrad}, by omitting the residual term we avoid noisy updates during the calibration phase, resulting in a more stable calibration process.


\input{tab/appendix_dpm.tex}
\section{Evaluation with advanced sampler}
In this section, we report additional results for the advanced sampler~(\ie, 3rd-order DPM-Solver++~\cite{lu2022dpmsolver}). We have already reported performance for Stable Diffusion~\cite{rombach2022high} with the PNDM sampler~\cite{liu2022pseudo} in Table.~\ref{tab:text_cond}. Here, we show in Table.~\ref{tab:dpm_solver} a quantitative comparisons between our method and Q-Diffusion~\cite{li2023q} for unconditional CIFAR-10 generation~\cite{krizhevsky2009learning} over 50 denoising steps. For quantization, we devide the 50-step denoising process into 17 groups: the first 16 groups contain three consecutive steps each, and the final group contains two steps. 
We observe that our method consistently outperforms Q-Diffusion~\cite{li2023q} in both FID~\cite{heusel2017gans} and FID2FP32~\cite{tang2025post}, demonstrating robustness across different samplers. Notably, in the 4/6-bit setting, our approach yields substantial gains, indicating enhanced tolerance to accumulated quantization error under low-bit activations.
In Fig.~\ref{fig:quali_dpm_suppl}, we present qualitative comparisons between our method and Q-Diffusion~\cite{li2023q} under 4/8-bit quantization. It demonstrates that our approach recovers visual fidelity close to the full-precision model, whereas Q-Diffusion~\cite{li2023q} produces visibly degraded outputs. This qualitative results further validates the ability of our method to mitigate accumulated quantization error.
\input{fig/quali_dpm_appendix.tex}


\section{Additional visualization on various benchmarks}
\vspace{-0.5mm}
In this section, we show additional qualitative results for unconditional image generation, class-conditional image generation and text-to-image generation. For unconditional image generation, we conduct the LSUN-Bedroom~\cite{yu2015lsun} using LDM-4~\cite{rombach2022high} with 200 denoising steps, and LSUN-Church~\cite{yu2015lsun} using LDM-8~\cite{rombach2022high} with 500 denoising steps. The model weights and activations are quantized to 3/8 bits respectively.  
As illustrated in Fig.~\ref{fig:quali_ldm_bedroom_suppl} and Fig.~\ref{fig:quali_ldm_church_suppl}, AccuQuant successfully prevents the accumulation of quantization errors, ensuring that generated images closely match their full precision counterparts with images containing rich semantics even in low-bit configurations.
For example, in Fig.~\ref{fig:quali_ldm_bedroom_suppl}, we observe that Q-Diffusion~\cite{li2023q} and TFMQ-DM~\cite{huang2024tfmq} present an overall monotonous coloration compared to the full precision results and generate different content of the bed due to the accumulated quantization error. In contrast, AccuQuant preserves a coloration and the content similar to that of the full precision model.
For class conditional image generation, we conduct the ImageNet~\cite{deng2009imagenet} using LDM-4~\cite{rombach2022high} with 20 denoising steps and quantized weights and activations to 3/8 bits respectively.
As illustrated in Fig.~\ref{fig:imagenet_comparison}, Q-Diffusion~\cite{li2023q} and TFMQ-DM~\cite{huang2024tfmq}, which do not account for accumulating quantization error, respectively exhibit chroma noise or produce monotone coloration. PTQD~\cite{he2023ptqd}, which does account for accumulating quantization error, generates vivid colors but alters content compared to full precision and producing unrealistic artifacts such as a chicken with two heads~(\textit{\ie, row 3, column 3 in Fig.~\ref{fig:imagenet_comparison}}). In contrast, AccuQuant generates vibrant colors, realistic imagery, and outputs that closely match those of the full precision model.
For text-to-image generation, we use COCO validation prompts~\cite{lin2014microsoft} in Fig.~\ref{fig:appendix_sd_coco_prompts} and user defined prompts in Fig.~\ref{fig:appendix_sd_user_prompts} with 50 denoising steps of Stable Diffusion v1.4~\footref{fn:sd} quantized into 4/8 bit-widths.
As illustrated in Fig.~\ref{fig:appendix_sd_coco_prompts}, PCR~\cite{tang2025post}, which is designed to mitigate accumulating quantization error, allocates more bit-width to activations yet still produces images with altered style or distortion compared to the full precision model. In contrast, AccuQuant uses fewer quantizers and a lower bit-width than PCR~\cite{tang2025post} but effectively minimizes accumulated quantization error, generating realistic images that closely match those of the full precision model.
We also visualize generated images conditioned on user defined prompts. As illustrated in Fig.~\ref{fig:appendix_sd_user_prompts}, Q-Diffusion~\cite{li2023q} and PCR~\cite{tang2025post} generates output that differ from those of the full precision model and misalign with the text prompt~(\textit{\eg, No astronaut in row 2, column 2 and row 3, column 4 in Fig.~\ref{fig:astronaut}}), while AccuQuant align strongly with the prompts. In summary, AccuQuant not only achieves superior performance on quantitative evaluation metrics but also qualitatively generates images that most closely resemble full precision outputs among state-of-the-art methods, align strongly with the prompts, and exhibit naturalness and semantic richness, demonstrating the superiority of our framework.

\input{tab/appendix_calibration_computation.tex}
\input{tab/appendix_inference_computation.tex}
\input{tab/appendix_lightweightqat.tex}
\section{Computational cost and efficiency}
\label{sec:computation}
In this section, we provide a detailed analysis of computational cost and efficiency in terms of calibration and inference. In Tab.~\ref{tab:ddim_cifar_calib_overhead}, we compare AccuQuant with Q-Diffusion~\cite{li2023q} in terms of computational cost for calibration and the generation performance. We can see that AccuQuant achieves superior performance with shorter calibration time compared to Q-Diffusion. We note that although AccuQuant may require more computational cost for one loss calculation, it only requires 50 epochs per group. In contrast, Q-diffusion calibrates each layer and residual block for 5000 epochs. Although AccuQuant incurs a marginal increase in energy consumption, it delivers a favorable trade-off for real-world deployment.
In addition, we evaluate the inference efficiency of our quantized diffusion model against both Q-Diffusion and the full-precision baseline. Since the official PyTorch quantization API does not support bit-widths lower than 8, we quantize both weights and activations to 8 bits and measure the memory usage and runtime latency using ONNX Runtime with the Intel Xeon Gold 6226R CPU. As shown in Tab.~\ref{tab:r6_cpu_cost}, both quantized models achieve over a 3 times speedup compared to the FP model. Our method incurs a marginally higher latency (by less than 0.18\%) and larger model size (by 0.006 MB) compared to Q-Diffusion, which we attribute to the separate quantization parameters per group. We also compare in Tab.~\ref{tab:r7_qat_compare} AccuQuant with a lightweight QAT approach, EfficientDM~\cite{He_2024_ICLR}. We report the results both under the same resource constraints (denoted as EfficientDM*) and using the official training recipe~\footnote{\url{https://github.com/ThisisBillhe/EfficientDM}} with larger training data and longer training time (denoted as EfficientDM-Full). We find that under an identical setting, AccuQuant achieves substantially better performance than EfficientDM*, suggesting that QAT frameworks cannot converge sufficiently within limited resource budgets. Furthermore, although EfficientDM-Full benefits from extended training time and larger datasets, AccuQuant still outperforms it in terms of FID2FP32, demonstrating the effectiveness of our method. In summary, although our method marginally increases latency and model size compared to Q-Diffusion, the benefits of reduced calibration time and improved generation quality offer a favorable trade-off for practical deployment.

\input{tab/appendix_restoration.tex}
\input{tab/appendix_styletransfer.tex}
\input{tab/appendix_dit.tex}
\section{Expanding to various tasks and advanced models}
In this section, we demonstrate the generalization ability of AccuQuant by evaluating image restoration (\eg, Gaussian deblurring), style transfer, and applying to transformer-based diffusion models~\cite{Peebles_2023_ICCV}. 
For Gaussian deblurring, we leverage the pre-trained DDPG~\cite{Garber_2024_CVPR} model from the official GitHub repository~\footnote{\url{https://github.com/tirer-lab/DDPG}} on the CelebA dataset (256 $\times$ 256 resolution, 1K images)~\cite{Liu_2015_ICCV}, injecting noise with $\sigma_Y$ = 0.05. Also, we use 100 total timesteps with a group size of 5 and calibrate with 64 samples obtained from a full-precision model. In Tab.~\ref{tab:deblur}, AccuQuant consistently outperforms Q-Diffusion~\cite{li2023q} across both PSNR and LPIPS metrics, demonstrating its effectiveness in the restoration setting. For style transfer (Fig.~\ref{tab:style_transfer}), we use Stable Diffusion v1.4~\footnote{\url{https://huggingface.co/CompVis/stable-diffusion-v-1-4-original}} with the prompt \textit{'A cartoon style'} and evaluated on the COCO validation set~\cite{lin2014microsoft}, with the entire timestep of 35 using the DDIM sampler~\cite{song2020denoising}. Since ground-truth images are unavailable for style transfer, we evaluate by comparing to the outputs obtained from the full-precision model. Note that we compute style and content losses following~\cite{Gatys_2016_CVPR}, using feature maps from a VGG network~\cite{Simonyan_2015_ICLR}. In Tab.~\ref{tab:style_transfer}, AccuQuant outperforms all evaluated metrics, highlighting its robustness for diverse generative tasks beyond standard image synthesis. 
For transformer-based diffusion model~\cite{Peebles_2023_ICCV} adaptation, we compare AccuQuant to recent diffusion-focused quantization methods~\cite{shang2023post,huang2024tfmq} including diffusion-transformer based quantization~\cite{Wu_2024_NeurIPS} and advanced transformer quantization method~\cite{li2023repq}. We conduct experiments on the ImageNet dataset~\cite{deng2009imagenet} using the DiT-XL/2~\cite{Peebles_2023_ICCV} with 100 timesteps, under both without and with classifier-free guidance settings~\cite{Ho_2021_NeurIPSW}. As shown in Tab.~\ref{tab:dit48_cfg}, AccuQuant outperforms transformer-based, diffusion-focused, and even DiT-specific quantization methods, demonstrating that reducing the accumulating error across diffusion timesteps is the key factor for quantizing diffusion models. In summary, by designing the quantization methods at the diffusion framework level rather than for a specific diffusion architecture, AccuQuant generalizes to diverse tasks and diffusion models.


\input{fig/quali_bedroom_appendix.tex}
\input{fig/quali_church_appendix.tex}
\input{fig/quali_imagenet_appendix.tex}
\input{fig/quali_coco_appendix.tex}
\input{fig/quali_coco_appendix2.tex}


==> accuquant-neurips-cameraready-arxiv/tab/ablation_gradient.tex <==

\begin{wraptable}{r}{0.45\textwidth}
    \vspace{-4mm}
    \caption{Quantitative comparisons of AccuQuant with and without the gradient approximation. We quantize DDIM~\cite{song2020denoising} on CIFAR-10~\cite{krizhevsky2009learning} with group size 5.}
    \vspace{-3mm}
    \renewcommand{\arraystretch}{1.3}

    \label{tab:grad_approx}
    \begin{center}
    \begin{small}
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{ccc}
    \toprule
    \multirow{2}{*}{\textbf{Bits (W/A)}} & \multicolumn{2}{c}{\textbf{FID~$\downarrow$ / FID2FP32~$\downarrow$}} \\ \cline{2-3}
    & \multicolumn{1}{c}{w/o Approximation} & \multicolumn{1}{c}{w/ Approximation} \\
    \midrule
    6/6 & \phantom{0}6.13 / 4.02 & \textbf{5.79} / \textbf{3.30} \\
    4/8 & \phantom{0}5.26 / 2.32 & \textbf{4.75} / \textbf{1.15} \\
    4/6 & \phantom{0}7.21 / 5.18 & \textbf{7.07} / \textbf{3.94} \\
    3/8 & \phantom{0}9.72 / 5.34 & \textbf{9.03} / \textbf{5.15} \\
    3/6 &       10.26 / 7.80     & \textbf{9.89} / \textbf{6.69} \\
    \bottomrule
    \end{tabular}}
    \end{small}
    \end{center}
    \vspace{-5mm}
\end{wraptable}
    

==> accuquant-neurips-cameraready-arxiv/tab/ablation_gradminmax.tex <==
\newcommand{\smallmath}[1]{{\footnotesize$#1$}}

\newcommand{\decpm}[3]{%
  \shortstack[c]{#1.#2 \\ {\footnotesize$\pm$#3}}%
}

\newcommand{\deconly}[2]{%
  #1.#2%
}


\begin{table}[t]
\centering
\begin{minipage}{0.58\linewidth}
  \centering
  % \vspace{-1mm}
  \caption{Comparison of the full gradient ($\frac{\partial \tilde{x}_{t-1}}{\partial \tilde{x}_t}$), Jacobian term ($c_t\frac{\partial \tilde{\epsilon}_\theta(\tilde{x}_t,t)}{\partial \tilde{x}_{t}}$), and our approximation. We quantize DDIM~\cite{song2020denoising} with CIFAR-10~\cite{krizhevsky2009learning} under W4A8 settings and report the mean and the entire range of the gradient at every 20 timestep.}
  \label{tab:grad_minmax}
  \vspace{1mm}
  % \renewcommand{\arraystretch}{1.2}
  \small
  \setlength{\tabcolsep}{5pt}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
      \toprule
      \textbf{Timestep} & \textbf{100} & \textbf{80} & \textbf{60} & \textbf{40} & \textbf{20} \\
      \midrule
      \multirow{2}{*}{\large$\frac{\partial \tilde{x}_{t-1}}{\partial \tilde{x}_t}$} 
      & 1.0221 
      & 1.0586 
      & 1.0273 
      & 1.0082 
      & 1.0008 \\
      
      & \textbf{$\pm$0.112} 
      & \textbf{$\pm$0.059} 
      & \textbf{$\pm$0.034} 
      & \textbf{$\pm$0.034} 
      & \textbf{$\pm$0.071} \\
      \addlinespace[3pt]
      \multirow{2}{*}{\large$c_t\frac{\partial \tilde{\epsilon}_\theta(\tilde{x}_t,t)}{\partial \tilde{x}_{t}}$} 
      &
      -0.1236 
      & -0.0097 
      & -0.0015 
      & -0.0006 
      & -0.0002 \\
      & \textbf{$\pm$0.112} 
      & \textbf{$\pm$0.059} 
      & \textbf{$\pm$0.034} 
      & \textbf{$\pm$0.034} 
      & \textbf{$\pm$0.071} \\
      \midrule
      $\sqrt{\frac{\alpha_{t-1}}{\alpha_t}}$ 
      & ~1.1457 
      & ~1.0683 
      & ~1.0288 
      & ~1.0088 
      & ~1.0010 \\
      \bottomrule
      \end{tabular}}
\end{minipage}
\hfill
\begin{minipage}{0.37\linewidth}
  \centering
  \caption{Quantitative comparisons of AccuQuant with and without gradient approximation. We quantize DDIM~\cite{song2020denoising} on CIFAR-10~\cite{krizhevsky2009learning} with group size 5.}
  \label{tab:grad_approx}
  \vspace{3.4mm}
  \renewcommand{\arraystretch}{1.15}
  \small
  \resizebox{\linewidth}{!}{
  \begin{tabular}{ccc}
    \toprule
    \multirow{2}{*}{\textbf{Bits (W/A)}} & \multicolumn{2}{c}{\textbf{FID~$\downarrow$ / FID2FP32~$\downarrow$}} \\ \cline{2-3}
    & w/o Approx. & w/ Approx. \\
    \midrule
    6/6 & 6.13 / 4.02 & \textbf{5.79} / \textbf{3.30} \\
    4/8 & 5.26 / 2.32 & \textbf{4.75} / \textbf{1.15} \\
    4/6 & 7.21 / 5.18 & \textbf{7.07} / \textbf{3.94} \\
    3/8 & 9.72 / 5.34 & \textbf{9.03} / \textbf{5.15} \\
    3/6 & 10.26 / 7.80 & \textbf{9.89} / \textbf{6.69} \\
    \bottomrule
  \end{tabular}}
\end{minipage}
\vspace{-1mm}
\end{table}

==> accuquant-neurips-cameraready-arxiv/tab/ablation_groupgrad.tex <==
\begin{table}[t]
    \caption{Quantitative comparisons of AccuQuant with and without the gradient approximation via various group sizes. We quantize DDIM~\cite{song2020denoising} on CIFAR-10~\cite{krizhevsky2009learning} under a 4/8-bit setting.}
    \vspace{2mm}
    \centering
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{ccc}
    \toprule
    \multirow{2}{*}{Group size} & \multicolumn{2}{c}{FID~$\downarrow$ / FID2FP32~$\downarrow$} \\ \cline{2-3}
    & \multicolumn{1}{c}{w/o Approximation} & \multicolumn{1}{c}{w/ Approximation} \\
    \midrule
    ~~1 & 6.88 / 3.11 & 6.88 / 3.11 \\
    ~~5 & 5.26 / 2.32 & \textbf{4.75} / \textbf{1.15} \\
    10 & 5.27 / \textbf{1.62} & \textbf{5.07} / 1.88 \\
    25 & 5.73 / 1.49     & \textbf{5.24} / 1.49 \\
    \bottomrule
    \end{tabular}}
    \label{tab:ablation_groupgrad}
    \vspace{-3mm}
\end{table}


==> accuquant-neurips-cameraready-arxiv/tab/ablation_groupsize.tex <==

\begin{wrapfigure}{r}{0.45\textwidth}
    \vspace{-4mm}
    \begin{minipage}{\linewidth}
        \centering
        
        \captionof{table}{Quantitative comparisons of AccuQuant under a 6/6-bit setting with varying group size.}
        \label{tab:group_size}
        % \vspace{-1mm}
        \resizebox{0.97\linewidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            \textbf{Group size} & \textbf{IS~$\uparrow$} & \textbf{FID~$\downarrow$} & \textbf{FID2FP32~$\downarrow$} \\
            \midrule
            ~~~~1   & 9.17 & ~~6.96 & ~~5.62 \\
            ~~~~2   & 9.02 & ~~6.82 & ~~4.48 \\
            ~~~~5   & \textbf{9.18} & ~~\textbf{5.79} & ~~\textbf{3.30} \\
            ~~10  & 9.13 & ~~6.18 & ~~4.30 \\
            ~~50  & 8.69 & 14.52 & 14.19 \\
            100 & 7.86 & 50.11 & 57.96 \\
            \bottomrule
        \end{tabular}}
        \vspace{-3mm}
        % \captionof{figure}{Memory usage of AccuQuant with and without gradient approximation during calibration.}
    \end{minipage}
\end{wrapfigure}

==> accuquant-neurips-cameraready-arxiv/tab/sota_bedrooms.tex <==


\begin{table}[t]
    \caption{Quantitative comparisons of LDM-4~\cite{rombach2022high} for image generation on LSUN-Bedrooms~\cite{yu2015lsun}. W/A represents bit-widths of weights (W) and activations (A). Numbers in bold are the best performance.}
    \label{tab:bedrooms}
    \begin{center}
    \begin{small}
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{LSUN-Bedrooms}} & \multicolumn{3}{c}{FID~$\downarrow$ / sFID~$\downarrow$ / FID2FP32~$\downarrow$} & \\ \cline{2-5}
    \multicolumn{1}{c|}{} & 4/8 & 3/8 & 32/32 \\
    \midrule
    \multicolumn{1}{c|}{Q-Diffusion~\cite{li2023q}}      & 5.46 / \phantom{0}7.92 / \phantom{0}1.92  & 11.98 / 14.02 / 7.54 & \multirow{5}{*}{3.04 / 7.07 / 0.00} \\
    \multicolumn{1}{c|}{PTQD~\cite{}}                    & 5.94 / 15.16 / \phantom{0}0.00            & \phantom{0}6.46 / 17.04 / 0.00                   & \\
    \multicolumn{1}{c|}{TFMQ-DM~\cite{huang2024tfmq}}    & 7.33 / 12.68 / \phantom{0}4.59            & 11.32 / 11.62 / 7.64                          & \\
    \multicolumn{1}{c|}{TAC~\cite{yao2024timestep}}      & 4.94 / \phantom{00}--\phantom{00}  / \phantom{0}--\phantom{00}                   & \phantom{0}5.14 /    --  /    --                         & \\
    \multicolumn{1}{c|}{AccuQuant~(Ours)}                & \textbf{4.03} / \textbf{\phantom{0}7.81} / \textbf{\phantom{0}1.07}  & \textbf{\phantom{0}4.18} / \textbf{10.45} / \textbf{1.14}  & \\
    \bottomrule
    \end{tabular}}
    \end{small}
    \end{center}
    \vspace{-5mm}
\end{table}

==> accuquant-neurips-cameraready-arxiv/tab/sota_churches.tex <==


\begin{table}[t]
    \caption{Quantitative comparisons of LDM-8~\cite{rombach2022high} for image generation on LSUN-Churches~\cite{yu2015lsun}. W/A represents bit-widths of weights (W) and activations (A). Numbers in bold are the best performance.}
    \label{tab:churches}
    \begin{center}
    \begin{small}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{LSUN-Churches}} & \multicolumn{5}{c}{FID~$\downarrow$ / sFID~$\downarrow$ / FID2FP32~$\downarrow$} &  \\ \cline{2-6}
    \multicolumn{1}{c|}{} & 4/8 & 4/6 & 3/8 & 3/6 & 32/32 \\
    \midrule
    \multicolumn{1}{c|}{Q-Diffusion~\cite{li2023q}}      & 4.49 / \textbf{10.36} / 0.79 & 45.24 / 25.96 / 40.58 & 5.68 / 11.25 / 1.49 & 47.49 / 27.97 / 42.27 & \multirow{5}{*}{3.91 / 10.10 / 0.00} \\
    \multicolumn{1}{c|}{PTQD~\cite{}}                    & 8.41 / TODO / TODO           & ---       & 12.68 / TODO / TODO  & ---       & \\
    \multicolumn{1}{c|}{TFMQ-DM~\cite{huang2024tfmq}}    & 8.43 / 19.83 / 10.14         & 8.60 / 20.77 / 10.07   & 9.03 / 21.77 / 10.48 & 9.84 / 14.20 / 10.19   & \\
    \multicolumn{1}{c|}{TAC~\cite{yao2024timestep}}      & \textbf{3.81} / -- / --      & ---       & 7.78 / -- / --       & ---       & \\
    \multicolumn{1}{c|}{AccuQuant~(Ours)}                & 3.99 / 10.67 / \textbf{0.66} & \textbf{7.47} / \textbf{11.07} / \textbf{4.84} & \textbf{5.04} / \textbf{11.07} / \textbf{1.26} & \textbf{8.91} / \textbf{12.58} / \textbf{5.79} & \\
    \bottomrule
    \end{tabular}}
    \end{small}
    \end{center}
    \vspace{-5mm}
\end{table}

==> accuquant-neurips-cameraready-arxiv/tab/sota_cifar.tex <==


\begin{table}[!t]
    \sisetup{
    detect-weight   = true,  
    detect-family   = true,   
    mode            = text,  
    }
    \centering
    \scriptsize
    \setlength{\tabcolsep}{2pt}  
    \caption{Quantization results for unconditional image generation on CIFAR-10 ($32\times32$)~\cite{krizhevsky2009learning}, LSUN-Churches ($256\times256$) and LSUN-Bedrooms ($256\times256$)~\cite{yu2015lsun}. $\dagger$: The official implementation of TFMQ-DM uses a 32-bit for certain layers, such as attention modules. We modified these components, such that all layers are quantized with the same bit-width, for fair comparisons with other methods. TAC~\cite{yao2024timestep} does not provide source codes, and thus its performance cannot be measured.}
    \vspace{3mm}
    \label{tab:uncond}
    %
    \begin{subtable}[t]{0.49\textwidth}
        \centering
        % \vspace{-1mm}

        \renewcommand{\arraystretch}{1.4}  

        \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}c l c S[table-format=1.2] S[table-format=2.2] S[table-format=2.2]@{}}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Bits(W/A)} & \textbf{IS}$\uparrow$ & \textbf{FID}$\downarrow$ & \textbf{FID2FP32}$\downarrow$ \\
        \midrule
        % \multirow{19}{*}{\parbox{2.2cm}{DDIM\\CIFAR-10\\(steps=100)}} 
        \multirow{21}{*}{\parbox{1.8cm}{\centering DDIM\\CIFAR-10\\(steps=100)}} 
            & Full-Precision                    & 32/32 &  9.09 &  4.26 &  0.00 \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  6/6  &  8.63 & 30.46 & 35.24 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  6/6  &  8.94 &  7.84 &  3.64 \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}6/6  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{9.18} &\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{5.79} &\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{3.30} \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  4/8  &  9.12 &  4.93 &  3.26 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  4/8  &  8.89 &  5.52 &  1.52 \\
            & TAC~\cite{yao2024timestep}        &  4/8  & \bfseries\tablenum{9.15} &  4.89 &    {{--}} \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}4/8  & \cellcolor[HTML]{ECF9FF}9.06 &\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{4.75} &\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{1.15} \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  4/6  & \bfseries\tablenum{9.47} & 25.35 & 30.66 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  4/6  &  9.15 & 11.04 &  7.39 \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}4/6  & \cellcolor[HTML]{ECF9FF}8.99 & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{7.07} &\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{3.94} \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  3/8  &  8.53 & 17.31 & 13.94 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  3/8  &  8.40 & 28.47 & 26.96 \\
            & TAC~\cite{yao2024timestep}        &  3/8  & \bfseries\tablenum{8.86} & 9.55 &    {{--}} \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}3/8  & \cellcolor[HTML]{ECF9FF}8.76 & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{9.03} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{5.15} \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  3/6  &  7.51 & 40.94 & 42.74 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  3/6  &  8.34 & 29.29 & 27.11 \\
            & TAC~\cite{yao2024timestep}        &  3/6  &  8.27 & 31.88 &    {{--}} \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}3/6  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{8.65} &\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{9.89} &\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{6.69} \\
        \bottomrule
        \end{tabular}
        }
    \end{subtable}%
    \hfill
    %
    \begin{subtable}[t]{0.49\textwidth}
        \centering
        % \vspace{-1mm}

        {\tiny                   
        \renewcommand{\arraystretch}{1.035} 
        \resizebox{\linewidth}{!}{
        \begin{tabular}{@{}c l c S S S@{}}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Bits(W/A)} & \textbf{FID}$\downarrow$ & \textbf{sFID}$\downarrow$ & \textbf{FID2FP32}$\downarrow$ \\ 
        \midrule
        \multirow{21}{*}{\parbox{1.5cm}{\centering LDM-8\\LSUN-Churches\\(steps=500)}} 
            & Full-Precision                    & 32/32 &  3.91 & 10.10 &  0.00 \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  4/8  &  4.49 & \bfseries\tablenum{10.36} &  0.79 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  4/8  &  8.43 & 19.83         & 10.14 \\
            & TAC~\cite{yao2024timestep}        &  4/8  & \bfseries\tablenum{3.81} & {--}            & {--}    \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}4/8  &  \cellcolor[HTML]{ECF9FF}3.99 & \cellcolor[HTML]{ECF9FF}10.67         & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{0.66} \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  4/6  & 45.24 & 25.96         & 40.58 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  4/6  &  8.60 & 20.77         & 10.07 \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}4/6  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{7.47} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{11.07}& \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{4.84} \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  3/8  &  5.68 & 11.25         &  1.49 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  3/8  &  9.03 & 21.77         & 10.48 \\
            & TAC~\cite{yao2024timestep}        &  3/8  &  7.78 & {--}            & {--}    \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}3/8  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{5.04} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{10.95}& \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{1.26} \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  3/6  &  47.49 & 27.97        &  42.27 \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  3/6  &  9.84  & 14.20        & 10.19 \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}3/6  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{8.91} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{12.58}& \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{5.79} \\
        \midrule
        \multirow{11}{*}{\parbox{1.5cm}{\centering LDM-4\\LSUN-Bedrooms\\(steps=200)}} 
            & Full-Precision                    & 32/32 &  3.04 &  7.07 & 0.00  \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  4/8  &  5.46 &  7.92 & 1.92  \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  4/8  &  7.33 & 12.68 & 4.59  \\
            & TAC~\cite{yao2024timestep}        &  4/8  &  4.94 & {--}    & {--}    \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}4/8  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{4.03} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{7.81} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{1.07} \\
        \cmidrule(lr){2-6}
            & Q-Diffusion~\cite{li2023q}        &  3/8  & 11.98 & 14.02 & 7.54  \\
            & TFMQ-DM{$^\dagger$}~\cite{huang2024tfmq}      &  3/8  & 11.32 & 11.62 & 7.64  \\
            & TAC~\cite{yao2024timestep}        &  3/8  &  5.14 & {--}    & {--}    \\
            & \cellcolor[HTML]{ECF9FF}Ours                  &  \cellcolor[HTML]{ECF9FF}3/8  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{4.18} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{10.45} &\cellcolor[HTML]{ECF9FF} \bfseries\tablenum{1.14} \\
        \bottomrule
        \end{tabular}
        }
        } % end tiny & arraystretch

    \end{subtable}
    % \vspace{-1mm}

\end{table}


==> accuquant-neurips-cameraready-arxiv/tab/sota_coco.tex <==
\begin{table}[!t]
    \sisetup{
      detect-weight   = true,  
      detect-family   = true,   
      mode            = text,  
    }
    \centering
    \scriptsize
    \setlength{\tabcolsep}{6pt}  
    \caption{Quantization results for text-to-image generation on MS-COCO ($512\times512$)~\cite{lin2014microsoft}. MP:~Mixed-precision quantization.}
    \vspace{2mm}
    \label{tab:text_cond}
    \resizebox{0.9\linewidth}{!}{
      \begin{tabular}{@{}c l c S S S@{}}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Bits(W/A)} & \textbf{FID}$\downarrow$ & \textbf{FID2FP32}$\downarrow$ & \textbf{CLIP Score}$\uparrow$ \\
        \midrule
        \multirow{6}{*}{\parbox{2.2cm}{\centering Stable Diffusion v1.4\\MS-COCO\\(steps=50)}}
          & Full-Precision   & 32/32        & 27.50            & 0.00            & 26.46            \\
        \cmidrule(lr){2-6}
          & Q-Diffusion~\cite{li2023q}      & 4/8          & 27.87            & 20.42           & 26.15            \\
          & PTQ4DM~\cite{shang2023post}           & 4/8          & 25.64            & 17.73           & 26.25            \\
          & PCR~\cite{tang2025post}              & 4/8.1 (MP)   & 23.86            & 14.39           & 26.35            \\
          & PCR~\cite{tang2025post}              & 4/8.4 (MP)   & \bfseries\tablenum{22.04}   & 14.25           & 26.48            \\
          & \cellcolor[HTML]{ECF9FF}Ours             & \cellcolor[HTML]{ECF9FF}4/8          & \cellcolor[HTML]{ECF9FF}22.73            & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{10.99}  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{26.85}   \\
        \bottomrule
      \end{tabular}
    }
  \vspace{-2mm}

  \end{table}

==> accuquant-neurips-cameraready-arxiv/tab/sota_imagenet.tex <==
\begin{table}[!t]
    \sisetup{
      detect-weight   = true,  
      detect-family   = true,   
      mode            = text,  
    }
    \scriptsize
    \setlength{\tabcolsep}{3pt}  
    \caption{Quantization results for class-conditional image generation on ImageNet ($256\times256$)~\cite{deng2009imagenet}.}
    \vspace{2mm}
    \label{tab:class_cond}
    \centering
    \resizebox{0.9\linewidth}{!}{
      \begin{tabular}{@{}c l c S[table-format=2.2] S[table-format=2.2] S[table-format=3.2] S[table-format=2.2] S[table-format=1.4] S[table-format=2.4] S[table-format=1.4]@{}}
        \toprule
        \textbf{Model} & \textbf{Method} & \textbf{Bits(W/A)} & \textbf{FID}$\downarrow$ & \textbf{sFID}$\downarrow$ & \textbf{IS}$\uparrow$ & \textbf{FID2FP32}$\downarrow$ & \textbf{LPIPS}$\downarrow$ & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ \\
        \midrule
        \multirow{15}{*}{\parbox{1.2cm}{\centering LDM-4\\ImageNet\\(steps=20)}}
          & Full-Precision                   & 32/32 & 11.13               &  7.85               & 368.19              &  0.00               & 0.00         & 0.00         & 0.00        \\
        \cmidrule(lr){2-10}
        & Q-Diffusion~\cite{li2023q}    &  4/8  &  9.55               & 13.50               & 339.44      &  1.71               & 0.1912    & 23.6703   & 0.8391   \\
        & PTQD~\cite{he2023ptqd}        &  4/8  &  9.99              & 8.43               & \bfseries\tablenum{361.95}     &  0.84               & 0.1598    & 24.0672   & 0.8614   \\  
        & TFMQ-DM~\cite{huang2024tfmq}     &  4/8  &  9.80               &  \bfseries\tablenum{7.19}               & 358.38     &  1.25               & 0.1702    & 23.6309   & 0.8567   \\
          & \cellcolor[HTML]{ECF9FF}Ours                              & \cellcolor[HTML]{ECF9FF}4/8  & \cellcolor[HTML]{ECF9FF}\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{9.39}       & \cellcolor[HTML]{ECF9FF}7.41      & \cellcolor[HTML]{ECF9FF}356.48              & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{0.65}       &\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{0.1585} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{24.4338} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{0.8713} \\
        \cmidrule(lr){2-10}
        & Q-Diffusion~\cite{li2023q}       &  3/8  &  7.57               & 12.43               & 266.65              & 11.26               & 0.3741    & 18.4588   & 0.6532   \\
        & PTQD~\cite{he2023ptqd}        &  3/8  &  7.75              & 9.51               & \bfseries\tablenum{308.47}     &  6.30               & 0.3446    & 19.2485   & 0.6728   \\    
        & TFMQ-DM~\cite{huang2024tfmq}     &  3/8  &  7.96               &  8.77               & 295.46              &  4.47               & 0.3942    & 16.8180   & 0.7200   \\
          & \cellcolor[HTML]{ECF9FF}Ours                              & \cellcolor[HTML]{ECF9FF}3/8  & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{6.61}       & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{8.65}       & \cellcolor[HTML]{ECF9FF}301.06     & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{3.86}       & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{0.2937} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{19.9392} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{0.7649} \\
        \cmidrule(lr){2-10}
        & Q-Diffusion~\cite{li2023q}       &  3/6  & 28.83               & 39.30               &  99.55              & 41.25               & 0.4666    & 17.9855   & 0.6358   \\
        & PTQD~\cite{he2023ptqd}          &  3/6  &  9.15              & 11.42               & 244.43     &  13.85               & 0.3852    & 18.1508   & 0.6662   \\    
        & TFMQ-DM~\cite{huang2024tfmq}     & 3/6  &  8.17               & 10.71               & 237.32              & 10.06               & 0.3928    & 17.4886   & 0.7183   \\
          & \cellcolor[HTML]{ECF9FF}Ours                              & \cellcolor[HTML]{ECF9FF}3/6  & \cellcolor[HTML]{ECF9FF}\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{5.95}       & \cellcolor[HTML]{ECF9FF}\cellcolor[HTML]{ECF9FF}\bfseries\tablenum{8.61}       & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{282.87}     & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{6.31}       & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{0.3296} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{19.0135} & \cellcolor[HTML]{ECF9FF}\bfseries\tablenum{0.7296} \\
        \bottomrule
      \end{tabular}
    }
  \vspace{-2mm}

  \end{table}

==> tab/ablation_gradient.tex <==

\begin{wraptable}{r}{0.45\textwidth}
    \vspace{-4mm}
    \caption{Quantitative comparisons of AccuQuant with and without the gradient approximation. We quantize DDIM~\cite{song2020denoising} on CIFAR-10~\cite{krizhevsky2009learning} with group size 5.}
    \vspace{-3mm}
    \renewcommand{\arraystretch}{1.3}

    \label{tab:grad_approx}
    \begin{center}
    \begin{small}
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{ccc}
    \toprule
    \multirow{2}{*}{\textbf{Bits (W/A)}} & \multicolumn{2}{c}{\textbf{FID~$\downarrow$ / FID2FP32~$\downarrow$}} \\ \cline{2-3}
    & \multicolumn{1}{c}{w/o Approximation} & \multicolumn{1}{c}{w/ Approximation} \\
    \midrule
    6/6 & \phantom{0}6.13 / 4.02 & \textbf{5.79} / \textbf{3.30} \\
    4/8 & \phantom{0}5.26 / 2.32 & \textbf{4.75} / \textbf{1.15} \\
    4/6 & \phantom{0}7.21 / 5.18 & \textbf{7.07} / \textbf{3.94} \\
    3/8 & \phantom{0}9.72 / 5.34 & \textbf{9.03} / \textbf{5.15} \\
    3/6 &       10.26 / 7.80     & \textbf{9.89} / \textbf{6.69} \\
    \bottomrule
    \end{tabular}}
    \end{small}
    \end{center}
    \vspace{-5mm}
\end{wraptable}
    

==> tab/sota_bedrooms.tex <==


\begin{table}[t]
    \caption{Quantitative comparisons of LDM-4~\cite{rombach2022high} for image generation on LSUN-Bedrooms~\cite{yu2015lsun}. W/A represents bit-widths of weights (W) and activations (A). Numbers in bold are the best performance.}
    \label{tab:bedrooms}
    \begin{center}
    \begin{small}
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{LSUN-Bedrooms}} & \multicolumn{3}{c}{FID~$\downarrow$ / sFID~$\downarrow$ / FID2FP32~$\downarrow$} & \\ \cline{2-5}
    \multicolumn{1}{c|}{} & 4/8 & 3/8 & 32/32 \\
    \midrule
    \multicolumn{1}{c|}{Q-Diffusion~\cite{li2023q}}      & 5.46 / \phantom{0}7.92 / \phantom{0}1.92  & 11.98 / 14.02 / 7.54 & \multirow{5}{*}{3.04 / 7.07 / 0.00} \\
    \multicolumn{1}{c|}{PTQD~\cite{}}                    & 5.94 / 15.16 / \phantom{0}0.00            & \phantom{0}6.46 / 17.04 / 0.00                   & \\
    \multicolumn{1}{c|}{TFMQ-DM~\cite{huang2024tfmq}}    & 7.33 / 12.68 / \phantom{0}4.59            & 11.32 / 11.62 / 7.64                          & \\
    \multicolumn{1}{c|}{TAC~\cite{yao2024timestep}}      & 4.94 / \phantom{00}--\phantom{00}  / \phantom{0}--\phantom{00}                   & \phantom{0}5.14 /    --  /    --                         & \\
    \multicolumn{1}{c|}{AccuQuant~(Ours)}                & \textbf{4.03} / \textbf{\phantom{0}7.81} / \textbf{\phantom{0}1.07}  & \textbf{\phantom{0}4.18} / \textbf{10.45} / \textbf{1.14}  & \\
    \bottomrule
    \end{tabular}}
    \end{small}
    \end{center}
    \vspace{-5mm}
\end{table}

==> tab/sota_churches.tex <==


\begin{table}[t]
    \caption{Quantitative comparisons of LDM-8~\cite{rombach2022high} for image generation on LSUN-Churches~\cite{yu2015lsun}. W/A represents bit-widths of weights (W) and activations (A). Numbers in bold are the best performance.}
    \label{tab:churches}
    \begin{center}
    \begin{small}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{LSUN-Churches}} & \multicolumn{5}{c}{FID~$\downarrow$ / sFID~$\downarrow$ / FID2FP32~$\downarrow$} &  \\ \cline{2-6}
    \multicolumn{1}{c|}{} & 4/8 & 4/6 & 3/8 & 3/6 & 32/32 \\
    \midrule
    \multicolumn{1}{c|}{Q-Diffusion~\cite{li2023q}}      & 4.49 / \textbf{10.36} / 0.79 & 45.24 / 25.96 / 40.58 & 5.68 / 11.25 / 1.49 & 47.49 / 27.97 / 42.27 & \multirow{5}{*}{3.91 / 10.10 / 0.00} \\
    \multicolumn{1}{c|}{PTQD~\cite{}}                    & 8.41 / TODO / TODO           & ---       & 12.68 / TODO / TODO  & ---       & \\
    \multicolumn{1}{c|}{TFMQ-DM~\cite{huang2024tfmq}}    & 8.43 / 19.83 / 10.14         & 8.60 / 20.77 / 10.07   & 9.03 / 21.77 / 10.48 & 9.84 / 14.20 / 10.19   & \\
    \multicolumn{1}{c|}{TAC~\cite{yao2024timestep}}      & \textbf{3.81} / -- / --      & ---       & 7.78 / -- / --       & ---       & \\
    \multicolumn{1}{c|}{AccuQuant~(Ours)}                & 3.99 / 10.67 / \textbf{0.66} & \textbf{7.47} / \textbf{11.07} / \textbf{4.84} & \textbf{5.04} / \textbf{11.07} / \textbf{1.26} & \textbf{8.91} / \textbf{12.58} / \textbf{5.79} & \\
    \bottomrule
    \end{tabular}}
    \end{small}
    \end{center}
    \vspace{-5mm}
\end{table}
